Automated design of quantum optical experiments for device-independent quantum key distribution

Device-independent quantum key distribution (DIQKD) reduces the vulnerability to side-channel attacks of standard QKD protocols by removing the need for characterized quantum devices. The higher security guarantees come however, at the price of a challenging implementation. Here, we tackle the question of the conception of an experiment for implementing DIQKD with photonic devices. We introduce a technique combining reinforcement learning, optimisation algorithm and a custom efficient simulation of quantum optics experiments to automate the design of photonic setups maximizing a given function of the measurement statistics. Applying the algorithm to DIQKD, we get unexpected experimental configurations leading to high key rates and to a high resistance to loss and noise. These configurations might be helpful to facilitate a first implementation of DIQKD with photonic devices and for future developments targeting improved performances.

==> Automated quantum optical experiment design for device-independent quantum keydistribution/data/perfect_data.tex <==
\sisetup{exponent-mode=scientific, output-exponent-marker = e, round-mode=places,round-precision=4, table-format=1.4}
\begin{table*}[htb]
	\small
    \centering
	\subfloat[][]{
    \begin{tabular}{@{}c|c|cccccccc@{}}
        \toprule
		$\eta$ & key rate & TMS$_{12}^r$ & TMS$_{12}^\theta$ & TMS$_{23}^r$ & TMS$_{23}^\theta$ & TMS$_{13}^r$ & TMS$_{13}^\theta$ & SMS$_2^r$ & SMS$_2^\theta$ \\
        \midrule
        0.0 & \num{0.9137156440435049} & \num{0.049722817215830654} & \num{1.5727154277819255} & \num{1.8764073632879066e-5} & \num{0.9894254331154752} & \num{1.856701335846047e-5} & \num{2.5610126545360554} & \num{-0.05117286572547441} & \num{0.011440006146520468}\\
        0.01 & \num{0.767686824245501} & \num{0.053057525168213125} & \num{1.572791980247873} & \num{0.00037044666908959994} & \num{0.9486749686882656} & \num{0.00036730617439308236} & \num{2.5192272913034697} & \num{-0.05210280697213371} & \num{0.004662270379311472}\\
        0.02 & \num{0.6527097562303206} & \num{0.05817602327926538} & \num{1.5700783994802932} & \num{0.00039093127753258173} & \num{0.9791425378771005} & \num{0.0003886551875928084} & \num{2.549291858704524} & \num{-0.052997503157831756} & \num{-0.00030360716706422173}\\
        0.03 & \num{0.5526583657839196} & \num{0.06372273262796384} & \num{1.5689454916528536} & \num{0.00042080877333334474} & \num{1.0055793496512315} & \num{0.0004187387705064189} & \num{2.5762350970436514} & \num{-0.053323098484885326} & \num{-0.007433092382639303}\\
        0.04 & \num{0.4631271062555493} & \num{0.07050382517622988} & \num{1.5730501478911978} & \num{0.000391120482662727} & \num{0.9869991590599775} & \num{0.00038950892008739034} & \num{2.5583004167843075} & \num{-0.054637094612921655} & \num{0.0073763314859287285}\\
        0.05 & \num{0.3818454061357336} & \num{0.07761142264418251} & \num{1.5706474404665152} & \num{0.0004228669947954165} & \num{1.0026923458886978} & \num{0.0004215177954348078} & \num{2.573535465207127} & \num{-0.05340299350861853} & \num{-0.00038425023527579227}\\
        0.06 & \num{0.3074375199825068} & \num{0.08550331788867509} & \num{1.570870860365692} & \num{0.00044169593857930876} & \num{1.0528150171944795} & \num{0.00044065762826705747} & \num{2.6235941111996004} & \num{-0.051199601182861466} & \num{0.0007461187634882162}\\
        0.07 & \num{0.23904644797744368} & \num{0.09418710759989403} & \num{1.5709843953975242} & \num{0.0005390418793262244} & \num{1.0958348373763576} & \num{0.0005381998231293484} & \num{2.6667227357832255} & \num{-0.04766083556698939} & \num{0.00017860510431416362}\\
        0.08 & \num{0.1762544562691568} & \num{0.10426362591863979} & \num{1.5707691780212856} & \num{0.0007960062434655799} & \num{1.109011082124043} & \num{0.0007951349759846516} & \num{2.679812520814698} & \num{-0.0436297306809708} & \num{-0.00023381535029516875}\\
        0.09 & \num{0.11926196626481445} & \num{0.11654109305761906} & \num{1.5709200564467434} & \num{0.0005839312848007497} & \num{1.1251317911601173} & \num{0.0005829915408562303} & \num{2.6959615654023006} & \num{-0.040095564032252444} & \num{0.0002930597945635898}\\
        0.1 & \num{0.06942244582532187} & \num{0.13162497243649987} & \num{1.5707821576658207} & \num{0.000623103962335954} & \num{1.144162309520832} & \num{0.0006211636182975314} & \num{2.7149738373740187} & \num{-0.03651855876528926} & \num{-0.00019758177371353864}\\
        0.102 & \num{0.060558227278010524} & \num{0.1349450098557854} & \num{1.5707585018512713} & \num{0.00052327903189517} & \num{1.104841830384577} & \num{0.0005214806261334437} & \num{2.6756204497940663} & \num{-0.03559399389404408} & \num{0.00011046840415571578}\\
        0.104 & \num{0.052132005416995586} & \num{0.13831957869586425} & \num{1.570838509049988} & \num{0.0005372365150406038} & \num{1.1237399902587446} & \num{0.0005352115867908647} & \num{2.6945731990640094} & \num{-0.03455160043271094} & \num{-0.00015647773388477416}\\
        0.106 & \num{0.04417876594296988} & \num{0.14173519784970728} & \num{1.570795984902848} & \num{0.0005553791998742446} & \num{1.1331624110867098} & \num{0.0005531220666390443} & \num{2.7039534069068885} & \num{-0.03338063552934783} & \num{1.1993887350053596e-5}\\
        0.108 & \num{0.03673446401658376} & \num{0.1451631198291172} & \num{1.5709719599939036} & \num{0.0004856025982853455} & \num{1.14839525791121} & \num{0.0004835003973559404} & \num{2.719275642911818} & \num{-0.032064383154082596} & \num{0.0003960858230979416}\\
        0.11 & \num{0.029835935177598305} & \num{0.14859466574937116} & \num{1.5708028684071953} & \num{0.0002915696467031814} & \num{1.1589434896667725} & \num{0.00029023848078715765} & \num{2.729830888994221} & \num{-0.03067571562234353} & \num{0.0011961491079098886}\\
        0.112 & \num{0.023520953524101995} & \num{0.15204954880216423} & \num{1.5709255785967369} & \num{0.0003560047563905937} & \num{1.1596446451484608} & \num{0.0003543583893804385} & \num{2.730472614848613} & \num{-0.02890531010016464} & \num{0.002212445255188961}\\
        0.114 & \num{0.017832038305403808} & \num{0.15541713031368432} & \num{1.5708413573159594} & \num{0.0005419738182360385} & \num{1.166925520457237} & \num{0.0005394327598318215} & \num{2.737764830022482} & \num{-0.02732976194882631} & \num{-0.0007121719014161614}\\
        0.116 & \num{0.012816553714857903} & \num{0.15881038048219676} & \num{1.5707930844439608} & \num{0.00026547023905303726} & \num{1.1814948639058773} & \num{0.0002642338658704905} & \num{2.7522358206565096} & \num{-0.02544338052134511} & \num{-0.00047822793100843084}\\
        0.118 & \num{0.008524427376769839} & \num{0.1621073357547439} & \num{1.5707735040394581} & \num{0.0002792909293397914} & \num{1.193727576335724} & \num{0.0002780003512710889} & \num{2.7645041811216307} & \num{-0.023568067954537773} & \num{-0.0007528299341258938}\\
        0.12 & \num{0.005016538228228229} & \num{0.1653552667706421} & \num{1.5710312300450988} & \num{0.0002952309040074982} & \num{1.205906773982519} & \num{0.00029391001647109796} & \num{2.7767573647047468} & \num{-0.02151504338893826} & \num{0.0006600415839161637}\\
        0.121 & \num{0.0035785376988395345} & \num{0.1669390939041563} & \num{1.570917713147816} & \num{0.0003089020471969722} & \num{1.2245585652360282} & \num{0.00030755901392759665} & \num{2.7954372625629733} & \num{-0.020587612570313905} & \num{-0.0008929105485063784}\\
        0.122 & \num{0.002364647591942992} & \num{0.16856203432956793} & \num{1.5710557106023526} & \num{0.0003234384706880014} & \num{1.2424696805967153} & \num{0.0003220596120985984} & \num{2.8132716021150106} & \num{-0.01954058129915898} & \num{0.00266699926583212}\\
        0.123 & \num{0.0013863516710328483} & \num{0.17007275839711888} & \num{1.5711260896316588} & \num{0.0003364655970811522} & \num{1.2582566789855276} & \num{0.0003350608815279443} & \num{2.8292645509200556} & \num{-0.018604427929916314} & \num{0.002119249925479024}\\
        0.124 & \num{0.000656548698126258} & \num{0.17160894911672453} & \num{1.5709909906244712} & \num{0.00035080047364590826} & \num{1.26929557243678} & \num{0.00034936504540068915} & \num{2.8401368373304936} & \num{-0.01798873566590311} & \num{0.007913210983791354}\\
        0.125 & \num{0.00018978825246385167} & \num{0.17307782327531593} & \num{1.5710851695160635} & \num{0.00036625756253021955} & \num{1.2814613728371942} & \num{0.000364747585425352} & \num{2.8522537477426546} & \num{-0.017036459301281} & \num{0.014553110658104187}\\
        0.126 & \num{2.858474128397681e-6} & \num{0.17436523301375673} & \num{1.5708141296925462} & \num{0.00010760292061526622} & \num{1.2278158736822509} & \num{0.00010716453501254617} & \num{2.7979361210256464} & \num{-0.015723791560569942} & \num{0.07660404899100497}\\
        0.1261 & \num{2.4878108340065097e-7} & \num{0.17426100159671037} & \num{1.5730711123190506} & \num{0.00010176682616025924} & \num{1.2163566272273465} & \num{0.00010132967871483578} & \num{2.78698109216216} & \num{-0.01742230883062528} & \num{0.10453563477040777}\\
        \bottomrule
    \end{tabular}
	}
	
    \subfloat[][]{
    \begin{tabular}{@{}c|c|ccccccccc@{}}
        \toprule
        $\eta$ & key rate & $A_0$: PS & $A_0$: D & $A_1$: SMS & $A_1$: D & $B_0$: D & $B_1$: SMS & $B_1$: D & $B_2$: D & $p$ \\
        \midrule
        0.0 & \num{0.9137156440435049} & \num{0.0015706998123422486} & \num{0.2223240376531575} & \num{-0.1949295183449991} & \num{-0.6304693917757955} & \num{-0.16790280938354915} & \num{0.2762770654504241} & \num{0.6847845192733076} & \num{0.2219942102550998} & \num{1.0e-9} \\
        0.01 & \num{0.767686824245501} & \num{0.00023369193425656123} & \num{0.23974632623830228} & \num{-0.19173218870510222} & \num{-0.6283938571004339} & \num{-0.16242911963504506} & \num{0.2852040689312475} & \num{0.7022821053638059} & \num{0.24114785898272503} & \num{-9.28730070638321e-10} \\
        0.02 & \num{0.6527097562303206} & \num{-0.0008048934306972955} & \num{0.26219710725766154} & \num{-0.184281078585384} & \num{-0.622986788359119} & \num{-0.1533367953630917} & \num{0.296632120008165} & \num{0.7266898999305361} & \num{0.264349381566493} & \num{2.323354252523758e-9} \\
        0.03 & \num{0.5526583657839196} & \num{-0.0002354071286790556} & \num{0.2840263257088412} & \num{-0.1777998485651183} & \num{-0.6197614157966962} & \num{-0.1453724702726128} & \num{0.30613514698186206} & \num{0.7489046962490405} & \num{0.28736397404912545} & \num{1.1074422575580379e-8} \\
        0.04 & \num{0.4631271062555493} & \num{0.0008933282207401874} & \num{0.30692116437119443} & \num{-0.17053955446657834} & \num{-0.6175027007275433} & \num{-0.13719574217883967} & \num{0.31607453068736685} & \num{0.771648159424396} & \num{0.3112682196861349} & \num{2.0419157871744076e-7} \\
        0.05 & \num{0.3818454061357336} & \num{5.4204571426773796e-5} & \num{0.33158894781454473} & \num{-0.1626615449317551} & \num{-0.6152166114071772} & \num{-0.12793660691589417} & \num{0.3235869837069408} & \num{0.7947412171146364} & \num{0.33706924968212265} & \num{-6.057099222833355e-6} \\
        0.06 & \num{0.3074375199825068} & \num{6.920407984820129e-5} & \num{0.3572243887988451} & \num{-0.15410041000187233} & \num{-0.6137821294211249} & \num{-0.11854086638856262} & \num{0.3298229818160921} & \num{0.8181252306656703} & \num{0.3639028724801244} & \num{5.8981799070012005e-5} \\
        0.07 & \num{0.23904644797744368} & \num{0.00012173185316537349} & \num{0.38416170653331505} & \num{-0.14479256088679748} & \num{-0.6130811539807546} & \num{-0.10864601095694706} & \num{0.3343341132219597} & \num{0.8416689135852099} & \num{0.3922882776767931} & \num{-0.0003219168573253689} \\
        0.08 & \num{0.1762544562691568} & \num{-3.480308690937066e-5} & \num{0.4130542670675739} & \num{-0.13407338552921041} & \num{-0.6131309143747168} & \num{-0.09785442987137093} & \num{0.33794253089810655} & \num{0.8657890708535518} & \num{0.4230111461720822} & \num{-0.0013199645714249693} \\
        0.09 & \num{0.11926196626481445} & \num{3.912208867092202e-5} & \num{0.4449701571021186} & \num{-0.12094237137025769} & \num{-0.613733280206438} & \num{-0.08550457705605596} & \num{0.341636281072171} & \num{0.8914914420099667} & \num{0.45765863638823} & \num{-0.004852259506123988} \\
        0.1 & \num{0.06942244582532187} & \num{1.9935040990821876e-5} & \num{0.48152381663121135} & \num{-0.1042606867485539} & \num{-0.6144454512422117} & \num{-0.07029022347984129} & \num{0.34499210074197967} & \num{0.9195666798545383} & \num{0.4982602683758703} & \num{0.016935771538582257} \\
        0.102 & \num{0.060558227278010524} & \num{-9.627119167076703e-6} & \num{0.4893963555027374} & \num{-0.10046014668520369} & \num{-0.6145666079484461} & \num{-0.06684005411655773} & \num{0.34542281340576547} & \num{0.9254210007311069} & \num{0.507106111209019} & \num{0.021502754811021364} \\
        0.104 & \num{0.052132005416995586} & \num{5.2223619385928395e-5} & \num{0.4973583755952538} & \num{-0.09674847968481246} & \num{-0.6148567933820477} & \num{-0.06343370992722734} & \num{0.34572874064281106} & \num{0.9312496523708753} & \num{0.516094224794034} & \num{0.027154801280397815} \\
        0.106 & \num{0.04417876594296988} & \num{-2.6836974629667725e-5} & \num{0.5053873446130522} & \num{-0.092925280103019} & \num{-0.6151903346541182} & \num{-0.05991909551641155} & \num{0.34584645944157283} & \num{0.9370551628937265} & \num{0.5251694527490706} & \num{0.034114036468573854} \\
        0.108 & \num{0.03673446401658376} & \num{0.0001164435727344349} & \num{0.5134106412909385} & \num{-0.08927924681595166} & \num{-0.6157264351331588} & \num{-0.05655069602504228} & \num{0.3457178481033893} & \num{0.94271953657722} & \num{0.5342880961963881} & \num{0.04264633449512472} \\
        0.11 & \num{0.029835935177598305} & \num{0.00010766983695990267} & \num{0.5214566796458299} & \num{-0.08556123000475684} & \num{-0.6162735962745164} & \num{-0.05303614131812392} & \num{0.34557604254014335} & \num{0.9483391122470302} & \num{0.5434112900004443} & \num{0.05312376227810184} \\
        0.112 & \num{0.023520953524101995} & \num{-1.937745020801811e-6} & \num{0.5296304897210387} & \num{-0.0817499247732653} & \num{-0.6168312435213615} & \num{-0.04932236247695475} & \num{0.3449790081286149} & \num{0.9539427169120525} & \num{0.5527048502239588} & \num{0.06601325421508838} \\
        0.114 & \num{0.017832038305403808} & \num{5.9934335771380954e-5} & \num{0.5373462272869859} & \num{-0.07839274038562755} & \num{-0.6178736832035487} & \num{-0.046363185881606525} & \num{0.3444754186946367} & \num{0.9591908311498841} & \num{0.5615482412832251} & \num{0.08194652580629365} \\
        0.116 & \num{0.012816553714857903} & \num{-3.7850648876448177e-5} & \num{0.5452379122164293} & \num{-0.07485701532625791} & \num{-0.6188064654847756} & \num{-0.04304540520521788} & \num{0.34363504741302736} & \num{0.9644590407252646} & \num{0.5705832930548705} & \num{0.10191322609109721} \\
        0.118 & \num{0.008524427376769839} & \num{8.770527380338484e-6} & \num{0.5528224408770572} & \num{-0.07177534866792522} & \num{-0.6200628882873218} & \num{-0.04004216133057652} & \num{0.34271173378312736} & \num{0.9693795629111056} & \num{0.5792932792674979} & \num{0.1274109414757529} \\
        0.12 & \num{0.005016538228228229} & \num{0.00010671299231250295} & \num{0.5602677493856949} & \num{-0.06886521934043222} & \num{-0.621530709182866} & \num{-0.03722331863843543} & \num{0.34148268618058336} & \num{0.9740901899395871} & \num{0.5879379565810219} & \num{0.16088067944562626} \\
        0.121 & \num{0.0035785376988395345} & \num{0.00010696173645472561} & \num{0.5638683155415896} & \num{-0.06748310281195473} & \num{-0.6223518218039} & \num{-0.03589504935727844} & \num{0.3409756048920908} & \num{0.9763971725156196} & \num{0.5920436719389436} & \num{0.18197557751133733} \\
        0.122 & \num{0.002364647591942992} & \num{5.671962016932856e-5} & \num{0.5675133524657107} & \num{-0.06612585928200108} & \num{-0.6232575684386877} & \num{-0.03455737790199916} & \num{0.34023333048347426} & \num{0.9786344928813155} & \num{0.5963069566161034} & \num{0.20721000506420378} \\
        0.123 & \num{0.0013863516710328483} & \num{0.0002719267055640455} & \num{0.5709550845814816} & \num{-0.06486732242844513} & \num{-0.6240752625203966} & \num{-0.03327356989923889} & \num{0.3396713155060758} & \num{0.9807526835601155} & \num{0.6002866568014645} & \num{0.23803659656212695} \\
        0.124 & \num{0.000656548698126258} & \num{9.909893146642353e-5} & \num{0.5742383691821337} & \num{-0.06397341321741076} & \num{-0.6252108967903658} & \num{-0.03233365804495943} & \num{0.33941678354591404} & \num{0.9828867764239125} & \num{0.6040667968756441} & \num{0.27752597354351677} \\
        0.125 & \num{0.00018978825246385167} & \num{-0.00019150693639799512} & \num{0.5776180103478544} & \num{-0.06385418751451902} & \num{-0.6266901035770444} & \num{-0.03161109624997573} & \num{0.33896605933127477} & \num{0.9849118705817328} & \num{0.6082119723385566} & \num{0.33330320677004005} \\
        0.126 & \num{2.858474128397681e-6} & \num{-0.0007799723075566727} & \num{0.5803588521837642} & \num{-0.06280274853011852} & \num{-0.627742654057401} & \num{-0.03050058625638148} & \num{0.3375102392225577} & \num{0.9863339626406665} & \num{0.611701087468242} & \num{0.44007795192682914} \\
        0.1261 & \num{2.4878108340065097e-7} & \num{0.00048656634548517656} & \num{0.5797017111214956} & \num{-0.06267569878282321} & \num{-0.6269875470730262} & \num{-0.029760494051951525} & \num{0.33944750702384874} & \num{0.9866304777049558} & \num{0.6110339633185572} & \num{0.47139568286852507} \\
        \bottomrule
    \end{tabular}
    }
    \centering
    \caption{Key rate and optical devices parameters for the circuit depicted in Fig.~\ref{fig:setup_eff_1} for different losses value $\eta$ considered to be the same for all NPNR-photon detectors. Parameters are for (a) state generation parameters (b) measurement settings. Single- and two-mode squeezers have two parameters $r,\theta$ which are given in separate column with name containing $r$ and $\theta$ as exponent. $p$ denotes the noisy pre-processing probability.}
	\label{tab:eff_1}
\end{table*}

==> Automated quantum optical experiment design for device-independent quantum keydistribution/data/robust_data.tex <==
\begin{table*}[htb]
    \centering
    \begin{tabular}{@{}c|c|ccccccccc@{}}
        \toprule
        $\eta$ & key rate & TMS$^r$ & TMS$^\theta$ & $A_0$: D$^x$ & $A_1$: SMS & $A_1$: D$^x$ & $B_0$: D$^p$ & $B_1$: D$^p$ & $B_2$: D$^p$ & $p$ \\
        \midrule
       0.0 & \num{0.46009387210564645} & \num{0.7417000768957924} & \num{1.570839830641258} & \num{0.02377876999573749} & \num{-0.3122462926177551} & \num{-0.7999602054055088} & \num{0.2925453939657808} & \num{-0.38842191033081436} & \num{-0.02066158508280264} & \num{3.6645065066271894e-9} \\
        0.01 & \num{0.3924638582073967} & \num{0.7267044973935837} & \num{1.5707901218430695} & \num{0.03350217887156588} & \num{-0.3116830187362099} & \num{-0.7914086656428623} & \num{0.28420636873321775} & \num{-0.39874190215082045} & \num{-0.029351192478674088} & \num{2.102086312261974e-5} \\
        0.02 & \num{0.3355692183226996} & \num{0.7111455591510221} & \num{1.5707912632985428} & \num{0.034711205066284424} & \num{-0.3133535925377775} & \num{-0.7939831125687918} & \num{0.2830388130753859} & \num{-0.4008288643481947} & \num{-0.02997778814417227} & \num{0.00016367314057320873} \\
        0.03 & \num{0.284114881611241} & \num{0.6931088853766729} & \num{1.570830504764672} & \num{0.03480560825067238} & \num{-0.31546054416536146} & \num{-0.7975897135149203} & \num{0.28216311552880213} & \num{-0.4015189335485504} & \num{-0.029529167168821004} & \num{-0.0005862341466553439} \\
        0.04 & \num{0.23708460097593353} & \num{0.6719509192475683} & \num{1.5708231127778154} & \num{0.03432481704977402} & \num{-0.31768420374513223} & \num{-0.8011785024075032} & \num{0.28087659200178905} & \num{-0.40114780424521246} & \num{-0.028495968877045048} & \num{0.0014921127552317492} \\
        0.05 & \num{0.1941927581225208} & \num{0.6469347749832935} & \num{1.5707699852855503} & \num{0.03343332095563525} & \num{-0.32004919684270666} & \num{-0.8043443662829997} & \num{0.27863398718588595} & \num{-0.3997538983056988} & \num{-0.02699724473316053} & \num{-0.0031228772714421036} \\
        0.06 & \num{0.1554552938093603} & \num{0.6177000482591506} & \num{1.5708080402964546} & \num{0.032268918938234796} & \num{-0.32235932625545993} & \num{-0.806444467969606} & \num{0.2749489872947484} & \num{-0.3972722080058082} & \num{-0.02518567967328743} & \num{0.00575116750904362} \\
        0.07 & \num{0.12103088228206094} & \num{0.5838392720398357} & \num{1.570779012306884} & \num{0.030851100511420294} & \num{-0.32452265626107435} & \num{-0.8072027880116769} & \num{0.26936271685463475} & \num{-0.3932832528669663} & \num{-0.0230426654739801} & \num{0.00963533699986678} \\
        0.08 & \num{0.09112026719657385} & \num{0.5453297125694256} & \num{1.5707544173984824} & \num{0.029309057595758473} & \num{-0.32625741818669574} & \num{-0.8057921494979312} & \num{0.2611303048673255} & \num{-0.3876684320481515} & \num{-0.020728547774400207} & \num{0.015053971242533937} \\
        0.09 & \num{0.06587876808081983} & \num{0.5024424985687558} & \num{1.5708315737780572} & \num{0.02757323746676478} & \num{-0.3271411899371896} & \num{-0.8017645464701091} & \num{0.24983548010447298} & \num{-0.3799018580857866} & \num{-0.018173851984017098} & \num{0.022276778338882093} \\
        0.1 & \num{0.04533808875524736} & \num{0.45579488776630017} & \num{1.5708053956692622} & \num{0.025683760813348517} & \num{-0.32673963462730987} & \num{-0.7943736114343984} & \num{0.2349135802709727} & \num{-0.36943765156832536} & \num{-0.015524834845498442} & \num{0.03154064435826958} \\
        0.11 & \num{0.029349988270456873} & \num{0.4061030925435241} & \num{1.570820839290217} & \num{0.023558623989765503} & \num{-0.32433245078371936} & \num{-0.7828962171783246} & \num{0.21601468004039662} & \num{-0.3556766443544208} & \num{-0.012804241760518661} & \num{0.043135729087237014} \\
        0.12 & \num{0.017566059072469442} & \num{0.3541561743213891} & \num{1.5708629093913724} & \num{0.021184324831322522} & \num{-0.31911897046329407} & \num{-0.7661916095080588} & \num{0.19294936203642704} & \num{-0.33788851618722304} & \num{-0.010095120513637994} & \num{0.0575837498064742} \\
        0.13 & \num{0.00945780491499737} & \num{0.3006994382305477} & \num{1.5706978044473856} & \num{0.01841540685245236} & \num{-0.31025755970588703} & \num{-0.74333119313314} & \num{0.1659026894290832} & \num{-0.31523378740212715} & \num{-0.007461662111265951} & \num{0.07573615879348464} \\
        0.14 & \num{0.004367574726555135} & \num{0.24608771828782502} & \num{1.570796614081143} & \num{0.015200055413917115} & \num{-0.29614212055074507} & \num{-0.7121564835017425} & \num{0.13523977020163064} & \num{-0.28646867195150816} & \num{-0.005057933981979447} & \num{0.09917055111819491} \\
        0.15 & \num{0.001573089550898188} & \num{0.1904258184565963} & \num{1.5707237510888146} & \num{0.011506510490320187} & \num{-0.2752444103453177} & \num{-0.6703674279001478} & \num{0.10179864972504446} & \num{-0.2496440709528563} & \num{-0.00297204384519507} & \num{0.1311466977386621} \\
        0.16 & \num{0.0003492137092130365} & \num{0.1329128331243102} & \num{1.570762933583878} & \num{0.007265664249142323} & \num{-0.24497761392360987} & \num{-0.6138824262580264} & \num{0.06676169659115623} & \num{-0.2007869202209524} & \num{-0.0013031980558572492} & \num{0.18007795418383865} \\
        0.161 & \num{0.00028648431374311834} & \num{0.12690738525054207} & \num{1.5707849307359145} & \num{0.006814029914285867} & \num{-0.24117788689298722} & \num{-0.6068253799656692} & \num{0.06311200464763786} & \num{-0.19485335515030855} & \num{-0.001165744270708223} & \num{0.18631097973002614} \\
        0.162 & \num{0.00023197496458049471} & \num{0.12105387834704937} & \num{1.5703988974789527} & \num{0.006390348595795667} & \num{-0.23769087329645464} & \num{-0.6003954639305813} & \num{0.0597131026449628} & \num{-0.18875409456945927} & \num{-0.0010167494399187034} & \num{0.1932980597510728} \\
        0.163 & \num{0.00018505679440439238} & \num{0.11516688530073484} & \num{1.57073124132386} & \num{0.005959400613504912} & \num{-0.23351196430638552} & \num{-0.593029246611218} & \num{0.05621698145116907} & \num{-0.18270274895929164} & \num{-0.0009092938939685616} & \num{0.2008980740358195} \\
        0.164 & \num{0.00014510957790903056} & \num{0.1090388481817058} & \num{1.5707201327896672} & \num{0.005519892497724053} & \num{-0.22939305408135982} & \num{-0.5854641575535133} & \num{0.05268331401418812} & \num{-0.1761412029016295} & \num{-0.0008122758253907174} & \num{0.20849686498343156} \\
        0.165 & \num{0.00011152507841294401} & \num{0.10275828657890512} & \num{1.5710835177905167} & \num{0.005026995640331716} & \num{-0.2250717974546318} & \num{-0.5775924510798233} & \num{0.04903551750079719} & \num{-0.16902587305721248} & \num{-0.0006903102147790759} & \num{0.21760983976054776} \\
        0.166 & \num{8.370598813145502e-5} & \num{0.09628686859600435} & \num{1.5706724288209455} & \num{0.004563068899503225} & \num{-0.2205580917278957} & \num{-0.5696180899660244} & \num{0.04541445180305898} & \num{-0.16135161916440902} & \num{-0.0005931641602373663} & \num{0.2258650447644764} \\
        0.167 & \num{6.106414754258882e-5} & \num{0.09001455791420655} & \num{1.5710210919898335} & \num{0.004125573605417319} & \num{-0.2159530541640542} & \num{-0.5606839521163839} & \num{0.04183788086302287} & \num{-0.1540255158324142} & \num{-0.00050247707556567} & \num{0.23633017477963913} \\
        0.168 & \num{4.301978463838729e-5} & \num{0.0838747339798898} & \num{1.5707816966436443} & \num{0.00371925868620828} & \num{-0.211101621170394} & \num{-0.5522330553895619} & \num{0.03843930846271649} & \num{-0.14619637021041487} & \num{-0.0004485479016983688} & \num{0.2474669092689109} \\
        0.169 & \num{2.9019338242508574e-5} & \num{0.07683741058534747} & \num{1.5707780847291373} & \num{0.003194394554459478} & \num{-0.20594058161905843} & \num{-0.5419914664596466} & \num{0.03459992572672523} & \num{-0.1372152656419072} & \num{-0.0003327202943894967} & \num{0.25949879831102934} \\
        0.17 & \num{1.8506913159410665e-5} & \num{0.07004745525814918} & \num{1.5698651906824064} & \num{0.002811291293992149} & \num{-0.1998289445239373} & \num{-0.5316036654409902} & \num{0.030949804539799036} & \num{-0.1280819289893427} & \num{-0.0003009599953402368} & \num{0.2718584040941959} \\
        0.171 & \num{1.0951958658189653e-5} & \num{0.06274961000782792} & \num{1.5714929368730923} & \num{0.0023506346850121883} & \num{-0.19392755000361842} & \num{-0.5211856922683729} & \num{0.027192570902214743} & \num{-0.11761055495462057} & \num{-0.00016297767514758594} & \num{0.28703067022699186} \\
        0.172 & \num{5.832911937564411e-6} & \num{0.05578086837262367} & \num{1.5714742227759038} & \num{0.0018728407625518775} & \num{-0.18825064518325046} & \num{-0.510902320660556} & \num{0.02372172562006009} & \num{-0.10696657210224317} & \num{-0.0001289177386867914} & \num{0.306088723238542} \\
        0.173 & \num{2.647582093451284e-6} & \num{0.04793240602619408} & \num{1.5706289263391604} & \num{0.0015119668549804476} & \num{-0.1783713333092117} & \num{-0.4946898242574739} & \num{0.019848683420953295} & \num{-0.095389380711792} & \num{-9.721313196711933e-5} & \num{0.32487749901424606} \\
        0.174 & \num{9.19168633206624e-7} & \num{0.03850447860781037} & \num{1.5710967614554512} & \num{0.0010040826128650557} & \num{-0.17120308462642608} & \num{-0.4808685847846702} & \num{0.01546016737438238} & \num{-0.07919940823162692} & \num{-6.423261794932558e-5} & \num{0.35135109310686274} \\
        0.175 & \num{1.6980974582025965e-7} & \num{0.03205192147316328} & \num{1.572209243076593} & \num{0.0008032324465915477} & \num{-0.1703794848068441} & \num{-0.473689340434537} & \num{0.012677544214357815} & \num{-0.06697068246784109} & \num{1.102520335303405e-5} & \num{0.3950502382836251} \\
        0.1756 & \num{1.0870893296655026e-8} & \num{0.031382360419748935} & \num{1.5694489126080222} & \num{0.0006620202042259442} & \num{-0.16206032439412887} & \num{-0.45882170376078923} & \num{0.01208813771667306} & \num{-0.06812949239621328} & \num{-0.00019527681105952383} & \num{0.43388371177111495} \\
        \bottomrule
    \end{tabular}
	\caption{Key rate and optical devices parameters for the circuit depicted in Fig.~\ref{fig:best_setup} for different losses value $\eta$ considered to be the same for all NPNR-photon detectors.}
	\label{tab:robust}
	
\end{table*}

